Spatial Mat\'ern fields driven by non-Gaussian noise

The article studies non-Gaussian extensions of a recently discovered link between certain Gaussian random fields, expressed as solutions to stochastic partial differential equations (SPDEs), and Gaussian Markov random fields. The focus is on non-Gaussian random fields with Mat\'ern covariance functions, and in particular we show how the SPDE formulation of a Laplace moving average model can be used to obtain an efficient simulation method as well as an accurate parameter estimation technique for the model. This should be seen as a demonstration of how these techniques can be used, and generalizations to more general SPDEs are readily available.

==> figs/pdfhistogram.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,psfrag}
%    \begin{document}\input{pdfhistogram}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           15-Sep-2010 14:20:25
% eps bounding box:     8 cm x 4.9135 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.05}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.15}%
\psfrag{v05}[r][r]{0.2}%
\psfrag{v06}[r][r]{0.25}%
\psfrag{v07}[r][r]{0.3}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{pdfhistogram.eps}}%
\end{psfrags}%
%
% End pdfhistogram.tex


==> figs/pdfhistogram1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,psfrag}
%    \begin{document}\input{pdfhistogram1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           01-Apr-2011 16:20:55
% eps bounding box:     8 cm x 4.9135 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% xticklabels:
\psfrag{x01}[t][t]{-8}%
\psfrag{x02}[t][t]{-6}%
\psfrag{x03}[t][t]{-4}%
\psfrag{x04}[t][t]{-2}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{pdfhistogram1.eps}}%
\end{psfrags}%
%
% End pdfhistogram1.tex


==> figs/pdfhistogram2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,psfrag}
%    \begin{document}\input{pdfhistogram2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           01-Apr-2011 16:47:22
% eps bounding box:     8 cm x 4.9135 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{pdfhistogram2.eps}}%
\end{psfrags}%
%
% End pdfhistogram2.tex


==> figs/sim2d1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,psfrag}
%    \begin{document}\input{sim2d1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           12-May-2011 15:26:42
% eps bounding box:     16 cm x 9.7871 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
%
% zticklabels:
\psfrag{z01}[r][r]{-10}%
\psfrag{z02}[r][r]{0}%
\psfrag{z03}[r][r]{10}%
\psfrag{z04}[r][r]{20}%
\psfrag{z05}[r][r]{30}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{sim2d1.eps}}%
\end{psfrags}%
%
% End sim2d1.tex


==> figs/sim2d2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,psfrag}
%    \begin{document}\input{sim2d2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           01-Apr-2011 17:01:32
% eps bounding box:     8 cm x 4.9135 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{40}%
\psfrag{x03}[t][t]{60}%
\psfrag{x04}[t][t]{80}%
\psfrag{x05}[t][t]{100}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{30}%
\psfrag{v04}[r][r]{40}%
\psfrag{v05}[r][r]{50}%
\psfrag{v06}[r][r]{60}%
\psfrag{v07}[r][r]{70}%
\psfrag{v08}[r][r]{80}%
\psfrag{v09}[r][r]{90}%
\psfrag{v10}[r][r]{100}%
%
% zticklabels:
\psfrag{z01}[r][r]{0}%
\psfrag{z02}[r][r]{5}%
\psfrag{z03}[r][r]{10}%
\psfrag{z04}[r][r]{15}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{sim2d2.eps}}%
\end{psfrags}%
%
% End sim2d2.tex

